HireVAE: An Online and Adaptive Factor Model Based on Hierarchical and Regime-Switch VAE

Factor model is a fundamental investment tool in quantitative investment, which can be empowered by deep learning to become more flexible and efficient in practical complicated investing situations. However, it is still an open question to build a factor model that can conduct stock prediction in an online and adaptive setting, where the model can adapt itself to match the current market regime identified based on only point-in-time market information. To tackle this problem, we propose the first deep learning based online and adaptive factor model, HireVAE, at the core of which is a hierarchical latent space that embeds the underlying relationship between the market situation and stock-wise latent factors, so that HireVAE can effectively estimate useful latent factors given only historical market information and subsequently predict accurate stock returns. Across four commonly used real stock market benchmarks, the proposed HireVAE demonstrate superior performance in terms of active returns over previous methods, verifying the potential of such online and adaptive factor model.

==> sec/name.tex <==
\begin{table}
    \centering
    \small
    \begin{tabular}{lrcrrrrrr}
        \toprule
        Method  &  Algo &    Enc  &  rIC & rICIR & AR & IR & SR & MD  \\
        \midrule
        RVAE-v    & Rule &   \ding{55}  & 0.05     & 0.67       & 21.62   & 4.80          & 0.83       & 7.61 \\
        RVAE     & Clus &  \ding{55}  & 0.05          & 0.50       & 13.72   & 2.17          & 0.51       & 9.12 \\
        RCVAE-v  & Rule &  \ding{55}    & 0.04          & 0.38       & 14.85  & 2.78          & 0.60       &  7.24\\
        RCVAE    &  Clus & \ding{55}& 0.03          & 0.32       & 2.61   & 0.82          & 0.10       & 7.33 \\
        HiReVAE-v  &  Rule &\ding{51}     & 0.06          & 0.67       & 24.54    & 4.26          & 0.73       & 7.65 \\
        \textbf{HiReVAE}   & \textbf{AOL} & \ding{51}       & 0.07         & 0.73       & 28.02    & 4.64          & 0.76       & 7.96 \\
        \bottomrule
    \end{tabular}
    \caption{Ablation study on rule-based regime switch and adaptive method in terms of their predictive power and stock selection performance among all Chinese A shares.
    ``r-" is abbreviated of rank. ``-v" indicates regime switching based on rule-based algorithm.\zkcmt{Need fill in results from server 35 and 187}}
    \label{tab:ablation-regime}
\end{table}


\begin{table}
    \centering
    \begin{tabular}{llrrrrr}
        \toprule
    ID  & Method  & Reg. & Stk & Mkt. &  $\mathbf{m}$      & $\mathbf{z}$  \\
        \midrule
    \ding{172}&  VAE     & \ding{55} & \ding{51}& \ding{51} & \ding{55} & \ding{51}  \\
    \ding{173}& VAE-S    & \ding{55} & \ding{51}& \ding{55} & \ding{55} & \ding{51}   \\
    \ding{174}&  RVAE    & \ding{51} & \ding{51}& \ding{51} & \ding{55} & \ding{51}   \\
    %\ding{175}&  RVAE-S  & \ding{51} & \ding{51}& \ding{55} & \ding{55} & \ding{51}   \\
    \ding{175}&  CVAE     & \ding{55} & \ding{51}& \ding{51} & \ding{55} & \ding{51}    \\
    %\ding{177}& CVAE-G   & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{51}   \\
    \ding{176} & RCVAE   & \ding{51} & \ding{51}& \ding{51} & \ding{55} & \ding{51}   \\
    %\ding{179} & RCVAE-G  & \ding{51} & \ding{51} & \ding{55} & \ding{51} & \ding{51}   \\
    \ding{177} & HiVAE   & \ding{55} & \ding{51}& \ding{51} & \ding{51} & \ding{51}  \\
    %\ding{181} & HiVAE-G & \ding{55} & \ding{51} & \ding{51} & \ding{51}  \\
    \ding{178} &  HiReVAE  & \ding{51} & \ding{51}& \ding{51} & \ding{51} & \ding{51}    \\
    %\ding{183} & HiReVAE-G  & \ding{51} & \ding{51} & \ding{51} & \ding{51}    \\
        \bottomrule
    \end{tabular}
    \caption{The settings for the ablation study on the effectiveness of a different combination of components in HiReVAE.}
    \label{tab:ablation-hirevae}
\end{table}



\begin{itemize}
    \item \textbf{Linear} is a linear factor model derived from \cite{fama1992cross}, with average pooling on the sequential dimension.
    \item \textbf{GRU} \cite{chung2014empirical} is a factor model in which a GRU extracts the sequential features and, in conjunction with a linear layer, predicts future returns.
    \item \textbf{Trans} \cite{ding2020hierarchical} is a factor model based on Transformer.
    \item \textbf{MLP} \cite{levin1995stock} is the first non-linear factor model with multilayer perceptrons, where we equip it with a GRU to extract time-series features.
    \item \textbf{GAT} \cite{veličković2018graph} is a graph attention work with a fully connected stock graph.
    \item \textbf{IGAT} \cite{wei2022factor} is a GAT, based on a stock-industry graph where there is an edge between two nodes if two stocks belong to the same industry.
    \item \textbf{DMFM} \cite{wei2022factor}  is a deep multifactor model built on top of a stock graph.
    \item \textbf{VAE} \cite{duan2022factorvae} is a stock prediction method based on VAE that treats latent stock variables as the optimal factors thus learned.
    \item \textbf{CVAE} \cite{gu2021autoencoder} is a factor model with a conditional autoencoder.
\end{itemize}



\zkcmt{Describe the results in Table \ref{tab:portfolio}. [xxx] outperforms the other methods in evaluation of their predictive power.}
\begin{table*}%[]%[!htb]
  \centering
  \begin{tabular}{lrrrrrrrrrrrr}
    \toprule
    &\multicolumn{4}{c}{CSI 300}  &\multicolumn{4}{c}{CSI 500}   &\multicolumn{4}{c}{CSI 1000}                 \\
   % \cmidrule(r){2-5} \cmidrule(r){6-9} \cmidrule(r){10-13}
    Method     & AR$\uparrow$ &IR$\uparrow$ & SR$\uparrow$  & MMD $\downarrow$&  AR$\uparrow$ &IR$\uparrow$ & SR$\uparrow$ & MMD $\downarrow$ & AR$\uparrow$ &IR$\uparrow$ & SR$\uparrow$& MMD $\downarrow$\\
    \midrule
    Linear   & 11.94  &0.30 &*.** & *.**  & *.**  &*.** &*.** & *.**  & *.**  &*.** &*.** & *.**\\
    GRU   & 19.40  &0.60 &*.** & *.**  & *.**  &*.** &*.** & *.**  & *.**  &*.** &*.** & *.**\\
    MLP    & 23.04  &0.78 &*.** & *.**  & *.**  &*.** &*.** & *.**  & *.**  &*.** &*.** & *.**\\
    Trans  & 7.21  &0.18 &*.** & *.**  & *.**  &*.** &*.** & *.**  & *.**  &*.** &*.** & *.**\\
    GAT     & 5.77  &0.14 &*.** & *.**  & *.**  &*.** &*.** & *.**  & *.**  &*.** &*.** & *.**\\
    IGAT     & 12.67  &0.41 &*.** & *.**  & *.**  &*.** &*.** & *.**  & *.**  &*.** &*.** & *.**\\
    DMFM    & 3.16  &0.05 &*.** & *.**  & *.**  &*.** &*.** & *.**  & *.**  &*.** &*.** & *.**\\
    VAE     & 26.49  &0.82 &*.** & *.**  & *.**  &*.** &*.** & *.**  & *.**  &*.** &*.** & *.**\\
    CVAE     & \underline{27.78}  &\textbf{0.91} &*.** & *.**  & *.**  &*.** &*.** & *.**  & *.**  &*.** &*.** & *.**\\
    HiReVAE     & \textbf{30.89}  &\underline{0.89} &*.** & *.**  & *.**  &*.** &*.** & *.**  & *.**  &*.** &*.** & *.**\\

    \bottomrule
  \end{tabular}
  \caption{The comparison of portfolio performances over the period 2015 to mid-2022 (\textbf{best}/\underline{2nd best}). 
  \label{tab:portfolio}
  }
\end{table*}
